Provable Sim-to-real Transfer in Continuous Domain with Partial Observations

Sim-to-real transfer trains RL agents in the simulated environments and then deploys them in the real world. Sim-to-real transfer has been widely used in practice because it is often cheaper, safer and much faster to collect samples in simulation than in the real world. Despite the empirical success of the sim-to-real transfer, its theoretical foundation is much less understood. In this paper, we study the sim-to-real transfer in continuous domain with partial observations, where the simulated environments and real-world environments are modeled by linear quadratic Gaussian (LQG) systems. We show that a popular robust adversarial training algorithm is capable of learning a policy from the simulated environment that is competitive to the optimal policy in the real-world environment. To achieve our results, we design a new algorithm for infinite-horizon average-cost LQGs and establish a regret bound that depends on the intrinsic complexity of the model class. Our algorithm crucially relies on a novel history clipping scheme, which might be of independent interest.

==> iclr2023/regret.tex <==
%\section{Regret Bound of LQG-VTR}
%\label{sec: regret}

%In this section we present the regret bound of the LQG-VTR algorithm. It then naturally comes to the sim-to-real gap of $\pi_{\mathrm{RT}}$ (Theorem \ref{thm: gap_rt}) by the reduction argument (Section \ref{subsec: reduction}). We also provide a proof sketch, and discuss the implication of the theorem.


%\subsection{Boundness of the States}
%\label{subsec: boundness}

%Let $\mathcal{K}$ be the number of episodes of LQG-VTR, an appreciated property of LQG-VTR is that the states and observations encountered in the algorithm will be bounded.

%As a consequence, with probability $1 - \delta$ the action clipping procedure (Line \ref{alg: action_clipping} of Algorithm \ref{alg: lqg_vtr}) preserves $u_t = \tilde{u}_t$ for any $1 \leq t \leq H$ since we set $M_u = \bar{U}$.


%Intuitively the optimism property of $\gU_k$ holds because we use value target regression, similar to the one used in \citet{ayoub2020model}. The proof is deferred to Section \ref{sec: appendix_missproof5}.%We present Lemma \ref{lem: optimism} for the moment, and defer the proof by a few sections where we define function class $\gF$ formally.


 


\subsection{Value Target Regression}
\label{subsec: vtr}

Finally, everything is prepared to perform the value target regression on $\gF$ \citep{ayoub2020model}. Now that the functions in $\gF$ have bounded $\ell_\infty$ norm according to Lemma \ref{lem: definition_D}. We need to carefully design the radius $\beta$ (Algorithm \ref{alg: lqg_vtr}) of the high confidence set to ensure optimism (Lemma \ref{lem: optimism}). Our switching protocol also helps us to keep the number of episodes low. At last, we can show a corresponding regret combining all the techniques. The full proof can be found in Appendix \ref{sec: appendix_missproof5}.

%We present some technical lemmas. 

